The Service Academy Brigade Reassignment Problem

After the COVID pandemic, student leadership development within the brigade of midshipmen at the United States Naval Academy (USNA) was severely degraded due to reduced student interaction from isolation and remote learning. Brigade leadership decided that reassignment of some students from their previous companies to new companies could facilitate new leadership bonds for the next academic year. All students in the classes of 2023 and 2024 are reassigned from their previous companies to new companies with the Brigade Reassignment Problem (BRP). The first goal of BRP is to minimize the number of students reassigned to their current company. The second goal seeks to improve the homogeneity of each company in terms of average metrics defined by brigade leadership. We create three similar mathematical programming models to achieve different goals of the BRP. The first model focuses on the first goal and quickly obtains an optimal solution. A second model focuses on the second goal and obtains high-quality feasible solutions. A third model combines the two goals and obtains an optimal solution within seven hours. USNA leadership implemented results from the first model to reassign the classes of 2023 and 2024 to new companies for the next academic year.

==> Objective3-2024.tex <==
\centering
\begin{tabular}{|c|c|c|c|c|c|c|} 
%\hline
%\multicolumn{7}{|c|}{BRP-PAIRS: Class of 2024 Company-level Summary Statistics} \\ 
\hline
~                    & AOM    & MOM    & \% Male & \% White & PRT score & \%  from same previous company  \\ 
\hline
minimum              & 504.49 & 498.67 & 66.67   & 60.53    & 86.83     & 11.84                            \\ 
\hline
maximum              & 589.64 & 588.77 & 78.95   & 79.49    & 92.10     & 12.82                            \\ 
\hline
average              & 564.57 & 551.63  & 69.71    & 71.49     & 89.59      & 12.66                            \\ 
\hline
standard deviation   & 21.48  & 25.38  & 3.61    & 6.00     & 1.11      & 0.36                             \\ 
\hline
median               & 565.49 & 552.03 & 68.83   & 71.79    & 89.34     & 12.82                            \\
\hline
\end{tabular}
